Finite-time Stabilization of Circular Formations using Bearing-only Measurements

This paper studies decentralized formation control of multiple vehicles when each vehicle can only measure the local bearings of their neighbors by using bearing-only sensors. Since the inter-vehicle distance cannot be measured, the target formation involves no distance constraints. More specifically, the target formation considered in this paper is an angle-constrained circular formation, where each vehicle has exactly two neighbors and the angle at each vehicle subtended by its two neighbors is pre-specified. To stabilize the target formation, we propose a discontinuous control law that only requires the sign information of the angle errors. Due to the discontinuity of the proposed control law, the stability of the closed-loop system is analyzed by employing a locally Lipschitz Lyapunov function and nonsmooth analysis tools. We prove that the target formation is locally finite-time stable with collision avoidance guaranteed. The evolution of the vehicle positions in the plane is also characterized.

==> figures/figure_tikz_invariant_formation.tex <==
\subfloat[Original formation.]
{
\begin{tikzpicture}[scale=0.5]
    \coordinate (z1) at (0,0);
    \coordinate (z2) at (0,4);
    \coordinate (z3) at (5,4);
    \coordinate (z4) at (6.5,0);
    \draw (z1)--(z2)--(z3)--(z4)--cycle;
    \def\radius{10pt}
    \draw [fill=white](z1) circle [radius=\radius];
    \draw [fill=white](z2) circle [radius=\radius];
    \draw [fill=white](z3) circle [radius=\radius];
    \draw [fill=white](z4) circle [radius=\radius];
\end{tikzpicture}
}
%========================================================
\subfloat[After rigid body transformation.]
{
\begin{tikzpicture}[scale=0.5]
    % original formation
    \coordinate (z1) at (0,0);
    \coordinate (z2) at (0,4);
    \coordinate (z3) at (5,4);
    \coordinate (z4) at (6.5,0);
    \draw[densely dashed] (z1)--(z2)--(z3)--(z4)--cycle;
    \def\radius{10pt}
    \draw [fill=white,densely dashed](z1) circle [radius=\radius];
    \draw [fill=white,densely dashed](z2) circle [radius=\radius];
    \draw [fill=white,densely dashed](z3) circle [radius=\radius];
    \draw [fill=white,densely dashed](z4) circle [radius=\radius];

    % after rigid body transformation
    \begin{scope}[shift={(1.5,2.5)},rotate=-15]
    \coordinate (z1) at (0,0);
    \coordinate (z2) at (0,4);
    \coordinate (z3) at (5,4);
    \coordinate (z4) at (6.5,0);
    \end{scope}
    \draw (z1)--(z2)--(z3)--(z4)--cycle;
    \def\radius{10pt}
    \draw [fill=white](z1) circle [radius=\radius];
    \draw [fill=white](z2) circle [radius=\radius];
    \draw [fill=white](z3) circle [radius=\radius];
    \draw [fill=white](z4) circle [radius=\radius];
\end{tikzpicture}
}
\\
%========================================================
\subfloat[After scaling.]
{
\begin{tikzpicture}[scale=0.5]
    % original formation
    \coordinate (z1) at (0,0);
    \coordinate (z2) at (0,4);
    \coordinate (z3) at (5,4);
    \coordinate (z4) at (6.5,0);
    \draw[densely dashed] (z1)--(z2)--(z3)--(z4)--cycle;
    \def\radius{10pt}
    \draw [fill=white,densely dashed](z1) circle [radius=\radius];
    \draw [fill=white,densely dashed](z2) circle [radius=\radius];
    \draw [fill=white,densely dashed](z3) circle [radius=\radius];
    \draw [fill=white,densely dashed](z4) circle [radius=\radius];

    % after rigid body transformation
    \begin{scope}[scale around={1.4:(2.8,2.3)}] % (2.8,2.3) is the intersection of the diagonal lines
    \coordinate (z1) at (0,0);
    \coordinate (z2) at (0,4);
    \coordinate (z3) at (5,4);
    \coordinate (z4) at (6.5,0);
    \end{scope}
    \draw (z1)--(z2)--(z3)--(z4)--cycle;
    \def\radius{10pt}
    \draw [fill=white](z1) circle [radius=\radius];
    \draw [fill=white](z2) circle [radius=\radius];
    \draw [fill=white](z3) circle [radius=\radius];
    \draw [fill=white](z4) circle [radius=\radius];
\end{tikzpicture}
}
%========================================================
\subfloat[After edge parallel motion.]
{
\begin{tikzpicture}[scale=0.5]
    % original formation
    \coordinate (z1) at (0,0);
    \coordinate (z2) at (0,4);
    \coordinate (z3) at (5,4);
    \coordinate (z4) at (6.5,0);
    \draw[densely dashed] (z1)--(z2)--(z3)--(z4)--cycle;
    \def\radius{10pt}
    \draw [fill=white,densely dashed](z1) circle [radius=\radius];
    \draw [fill=white,densely dashed](z2) circle [radius=\radius];
    \draw [fill=white,densely dashed](z3) circle [radius=\radius];
    \draw [fill=white,densely dashed](z4) circle [radius=\radius];

    % after rigid body transformation
    \coordinate (z1) at (0,0);
    \coordinate (z2) at (0,4);
    \begin{scope}[xshift=1.5cm]
    \coordinate (z3) at (5,4);
    \coordinate (z4) at (6.5,0);
    \end{scope}
    \draw (z1)--(z2)--(z3)--(z4)--cycle;
    \def\radius{10pt}
    \draw [fill=white](z1) circle [radius=\radius];
    \draw [fill=white](z2) circle [radius=\radius];
    \draw [fill=white](z3) circle [radius=\radius];
    \draw [fill=white](z4) circle [radius=\radius];
\end{tikzpicture}
}
